SemiReward: A General Reward Model for Semi-supervised Learning

Semi-supervised learning (SSL) has witnessed great progress with various improvements in the self-training framework with pseudo labeling. The main challenge is how to distinguish high-quality pseudo labels against the confirmation bias. However, existing pseudo-label selection strategies are limited to pre-defined schemes or complex hand-crafted policies specially designed for classification, failing to achieve high-quality labels, fast convergence, and task versatility simultaneously. To these ends, we propose a Semi-supervised Reward framework (SemiReward) that predicts reward scores to evaluate and filter out high-quality pseudo labels, which is pluggable to mainstream SSL methods in wide task types and scenarios. To mitigate confirmation bias, SemiReward is trained online in two stages with a generator model and subsampling strategy. With classification and regression tasks on 13 standard SSL benchmarks across three modalities, extensive experiments verify that SemiReward achieves significant performance gains and faster convergence speeds upon Pseudo Label, FlexMatch, and Free/SoftMatch. Code and models are available at https://github.com/Westlake-AI/SemiReward.

==> Tabs/tab_ap_hypersettingaudio.tex <==
\begin{table}[H]
\centering
\caption{Hyper-parameters of Audio tasks.}
\resizebox{0.8\textwidth}{!}{\begin{tabular}{l|lll}
\hline
Dataset                 & UrbanSound8k             & FSDNoisy                   & ESC-50        \\
Sampling Rate & \multicolumn{3}{c}{16,000} \\
Max Length & 4.0 & 5.0 & 5.0 \\
Model                   & \multicolumn{3}{c}{HuBERT-Base}            \\
Weight Decay            & \multicolumn{3}{c}{5e-4}                                                     \\
Labeled Batch size      & \multicolumn{3}{c}{8}                                                       \\
Unlabeled Batch size    & \multicolumn{3}{c}{8}                                                       \\
Learning Rate           & 5e-4                     & 1e-4                     & 5e-5                   \\
Layer Decay Rate        & 0.75 & 0.75 & 0.85                    \\
Scheduler               & \multicolumn{3}{c}{$\eta = \eta_0 \cos(\frac{7\pi k}{16K})$}                 \\
Model EMA Momentum      & \multicolumn{3}{c}{0.999}                                                    \\
Prediction EMA Momentum & \multicolumn{3}{c}{0.999}                                                    \\
Weak Augmentation       & \multicolumn{3}{c}{Random Sub-sample}                      \\
\multirow{2}{*}{Strong Augmentation}     & \multicolumn{3}{c}{Random Sub-sample, Random Gain}\\
& \multicolumn{3}{c}{ Random Pitch, Random Speed}\\ \hline
\end{tabular}
}
\label{tab:ap_hypersettingaudio}
\end{table}


==> Tabs/tab_ap_hypersettingnlp.tex <==
\begin{table}[H]
\centering
\caption{Hyper-parameters of NLP tasks.}
\resizebox{0.8\textwidth}{!}{\begin{tabular}{c|ccc}
\hline
Dataset                 &  AG News & Yahoo! Answer & Yelp-5               \\
Max Length              & \multicolumn{3}{c}{512}                    \\
Model                   & \multicolumn{3}{c}{Bert-Base}           \\
Weight Decay            & \multicolumn{3}{c}{1e-4}                                                     \\
Labeled Batch size      & \multicolumn{3}{c}{4}                                                       \\
Unlabeled Batch size    & \multicolumn{3}{c}{4}                                                       \\
Learning Rate           &5e-4 &1e-4 &5e-5                   \\
Layer Decay Rate        & 0.65 & 0.65  & 0.75                    \\
Scheduler               & \multicolumn{3}{c}{$\eta = \eta_0 \cos(\frac{7\pi k}{16K})$}                 \\
Model EMA Momentum      & \multicolumn{3}{c}{0.999}                                                    \\
Prediction EMA Momentum & \multicolumn{3}{c}{0.999}                                                    \\
Weak Augmentation       & \multicolumn{3}{c}{None}                      \\
Strong Augmentation     & \multicolumn{3}{c}{Back-Translation \cite{xie2020unsupervised}} \\ \hline
\end{tabular}
}
\label{tab:ap_hypersettingnlp}
\end{table}
